High precision determination of $\alpha_s$ from a global fit of jet rates

We present state-of-the-art extractions of the strong coupling based on N$^3$LO+NNLL accurate predictions for the two-jet rate in the Durham clustering algorithm at $e^+e^-$ collisions, as well as a simultaneous fit of the two- and three-jet rates taking into account correlations between the two observables. The fits are performed on a large range of data sets collected at LEP and PETRA colliders, with energies spanning from $35$ GeV to $207$ GeV. Owing to the high accuracy of the predictions used, the perturbative uncertainty is considerably smaller than that due to hadronization. Our best determination at the $Z$ mass is $\alpha_s(M_Z) = 0.11881 \pm 0.00063(exp.) \pm 0.00101(hadr.) \pm 0.00045(ren.) \pm 0.00034(res.)$, which is in agreement with the latest world average and has a comparable total uncertainty.

==> Makefile <==
#ulimit -u 10000
latexfile=JRT
newname?=JRT
STYLE=jhep

LATEX=  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex  lineno.sty  mcite.sty  nicefrac.sty  supertabular.sty  units.sty
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex  mcite.sty  nicefrac.sty  supertabular.sty  units.sty
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex   
endif

ifeq ($(STYLE),jhep)
	STYLE_SPECIFIC_FILES=jheppub.sty $(latexfile)-jhep.tex JHEP.bst
endif


all: $(latexfile)-$(STYLE).pdf


tar:  Makefile figurelist-$(STYLE).txt $(constanttables) $(tables)  fitranges.tex  $(latexfile)-def.tex  $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
#	mkdir -p TAR/Tables
#	mkdir -p TAR/ConstantTables
	cp Makefile  fitranges.tex  $(latexfile).bst $(latexfile).bib  $(latexfile)-val.tex $(latexfile)-def.tex $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex    $(STYLE_SPECIFIC_FILES) TAR
#	cp $(constanttables) TAR/ConstantTables
#	cp $(tables) TAR/Tables
	for a in $$(cat   figurelist-$(STYLE).txt); do\
		cp $$a TAR/Figures;\
	done	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
ifeq ($(STYLE),jhep)
	rm TAR/$(newname).bst 
endif
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	mv TAR/$(latexfile)-val.tex TAR/$(newname)-val.tex
	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),jhep)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	cp TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname).bbl
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif

	tar -zcvf   $(newname).tar.gz -C TAR . 
	#rm -rf TAR


figures=

$(latexfile)-$(STYLE).fls: $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex  $(latexfile)-val.tex $(STYLE_SPECIFIC_FILES)
		pdflatex -recorder $(latexfile)-$(STYLE).tex
figurelist-$(STYLE).txt:  $(latexfile)-$(STYLE).fls
		cat $(latexfile)-$(STYLE).fls | grep pdf | grep Figures | sed 's@\./@@g' |sort | cut -f2 -d' '| uniq  > figurelist-$(STYLE).txt
tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex  $(latexfile)-val.tex $(STYLE_SPECIFIC_FILES)
	
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)


pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t  --add-tex-command="prog p" --add-tex-command="author p" --add-tex-command="institute p" --add-tex-command="text p" --add-tex-command="affil  p" --add-tex-command="Refrs p" --dont-tex-check-comments -d en_GB -c $$a ;\
		done

clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


split:
		rm -rf splitdir
		mkdir -p splitdir
		csplit JRT-fig.tex  --prefix=figsplit --suffix=%02d  "/newcommand/" "{*}" 
		for a in $$(ls -1 figsplit*); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		b=$$(cat $$a | grep newcommand | cut -f2 -d\{| cut -f1 -d\} | tr -d '\\'   );\
		mv $$a splitdir/$$b".tex";\
		done
merge: JRT-merged-fig.tex
JRT-merged-fig.tex:
		cat splitdir/*tex  > JRT-merged-fig.tex






